Fire Now, Fire Later: Alarm-Based Systems for Prescriptive Process Monitoring

Predictive process monitoring is a family of techniques to analyze events produced during the execution of a business process in order to predict the future state or the final outcome of running process instances. Existing techniques in this field are able to predict, at each step of a process instance, the likelihood that it will lead to an undesired outcome.These techniques, however, focus on generating predictions and do not prescribe when and how process workers should intervene to decrease the cost of undesired outcomes. This paper proposes a framework for prescriptive process monitoring, which extends predictive monitoring with the ability to generate alarms that trigger interventions to prevent an undesired outcome or mitigate its effect. The framework incorporates a parameterized cost model to assess the cost-benefit trade-off of generating alarms. We show how to optimize the generation of alarms given an event log of past process executions and a set of cost model parameters. The proposed approaches are empirically evaluated using a range of real-life event logs. The experimental results show that the net cost of undesired outcomes can be minimized by changing the threshold for generating alarms, as the process instance progresses. Moreover, introducing delays for triggering alarms, instead of triggering them as soon as the probability of an undesired outcome exceeds a threshold, leads to lower net costs.

==> threats.tex <==
\section{Limitations and Future Work}
\label{sec:threats}

While the scenarios discussed in Boxes~1-4 show that the proposed framework is versatile enough to cover a variety of cases, the current version of the framework relies on two main assumptions. First, it assumes that an alarm always triggers an intervention, thus ignoring that a process worker might in some cases decide not to or be unable to intervene. Additionally, the current version of the framework considers each case in isolation, omitting the overall workload of the process workers, which in reality is an important factor for determining the number of alarms that can be acted upon. This limitation can be lifted by, e.g., combining the alarm system with~\cite{CONFORTI20151}, which proposes a recommender system that optimizes suggestions in case of concurrent process executions. 

Next to this limitation, we acknowledge the importance of further investigation on the applicability of the framework in practice.
In particular, in the future, we aim at collaborating with companies and institutions to study whether process stakeholders are able to define the costs in a natural and simple way. Also, we plan to further investigate the consequences of incorrect and/or imprecise instantiations of the cost models.
Furthermore, the current evaluation is limited to measuring the benefit of the alarm system in an offline manner, while a more thorough evaluation would consist in deploying the alarming mechanism in a real organization and making an end-to-end comparison of the costs before and after the deployment of the alarm system. However, this is a difficult task for two main reasons. First, companies need to be willing to let the technique really influence the process executions. Second, the end-to-end effectiveness analysis cannot be conducted without coupling the alarm system with a recommender system: if the system raises proper alarms, but inappropriate interventions are taken, the system would still be ineffective.
Another avenue for future work is to extend the framework with active learning methods in order to incrementally tune the alarming mechanism based on feedback about the relevance of the alarms and the effectiveness of the interventions.




